Clues to the Nature of SN 2009ip II: The Continuing Photometric and Spectroscopic Evolution to 1000 Days

The 2012 brightening of SN 2009ip was dominated by emission from the interaction of ejecta with the surrounding circumstellar material (CSM) produced by episodic mass loss from the progenitor, complicating the diagnosis of whether the underlying explosion was a true supernova or a nonterminal eruption of a massive star. In this paper, we contribute a time series of optical photometric and spectroscopic observations for SN 2009ip from 1 to 3 years after the 2012 outburst, collected at the Las Cumbres Observatory and the Keck Observatory. We find that the brightness of SN 2009ip continues to decline with no deviations from a linear slope of $0.0030\pm0.0005$ $\rm mag\ day^{-1}$ in the $r^{\prime}$ band, and demonstrate that this is similar to both observations and models of CSM-ejecta interaction. We show that the late-time spectra continue to be dominated by the signature features of CSM interaction, and that the large ratio of $L_{\rm H\alpha}/L_{\rm H\beta}\approx40$ implies that the material remains optically thick to Balmer photons ("Case C" recombination). We combine our late-time photometry and spectra with early-time data for SN 2009ip and provide a comprehensive discussion that incorporates recently published models and observations for transient phenomena dominated by CSM-ejecta interaction, and conclude that the presence of broad H$\alpha$ at early times remains among the best evidence that a terminal supernova has occurred. Finally, we compare our late-time spectra to those of Type IIn SNe and SN impostors at late phases and find that although SN 2009ip has some similarities with both types, it has more differences with late-time impostor spectra.

==> tab1_full.tex <==
\begin{table}
\label{tab:phot}
\begin{tabular}{cccc}
\hline
\hline
\multicolumn{2}{c}{LCOGT $g$-band} & \multicolumn{2}{c}{LCOGT $r$-band}\\
MJD & Magnitude & MJD & Magnitude \\
\hline
56445 & $19.73\pm0.33$  & 56445 & $18.42\pm0.14$ \\
56447 & $19.30\pm0.49$  & 56446 & $18.37\pm0.20$ \\
56449 & $19.52\pm0.33$  & 56449 & $18.38\pm0.13$ \\
56456 & $19.93\pm0.28$  & 56452 & $18.75\pm0.22$ \\
56458 & $19.98\pm0.28$  & 56454 & $18.38\pm0.12$ \\
56462 & $19.78\pm0.24$  & 56458 & $18.52\pm0.16$ \\
56474 & $19.64\pm0.44$  & 56466 & $18.61\pm0.19$ \\
56479 & $19.77\pm0.32$  & 56468 & $18.83\pm0.46$ \\
56481 & $19.66\pm0.95$  & 56474 & $18.48\pm0.16$ \\
56483 & $19.99\pm0.40$  & 56475 & $18.51\pm0.13$ \\
56485 & $20.08\pm0.20$  & 56479 & $18.44\pm0.47$ \\
56486 & $19.92\pm0.33$  & 56481 & $18.59\pm0.22$ \\
56487 & $19.85\pm0.20$  & 56483 & $18.59\pm0.19$ \\
56489 & $19.88\pm0.58$  & 56485 & $18.69\pm0.16$ \\
56490 & $19.67\pm0.26$  & 56486 & $18.53\pm0.20$ \\
56491 & $19.76\pm0.31$  & 56487 & $18.60\pm0.15$ \\
56503 & $19.81\pm0.26$  & 56489 & $18.64\pm0.11$ \\
56504 & $19.43\pm0.30$  & 56490 & $18.60\pm0.14$ \\
56508 & $19.76\pm0.42$  & 56491 & $18.60\pm0.12$ \\
56512 & $19.82\pm0.22$  & 56498 & $18.57\pm0.33$ \\
56518 & $19.84\pm0.28$  & 56502 & $18.54\pm0.32$ \\
56520 & $20.05\pm0.57$  & 56503 & $18.62\pm0.15$ \\
56530 & $19.54\pm0.60$  & 56504 & $18.44\pm0.25$ \\
56534 & $20.30\pm0.66$  & 56508 & $18.56\pm0.18$ \\
56539 & $20.02\pm0.34$  & 56512 & $18.53\pm0.24$ \\
56540 & $19.57\pm0.23$  & 56518 & $18.80\pm0.20$ \\
56541 & $20.03\pm0.22$  & 56520 & $18.63\pm0.21$ \\
56544 & $19.95\pm0.29$  & 56524 & $19.05\pm0.38$ \\
56546 & $19.74\pm0.30$  & 56525 & $18.62\pm0.23$ \\
56558 & $19.76\pm0.51$  & 56528 & $18.90\pm0.17$ \\
56563 & $20.19\pm0.25$  & 56530 & $18.80\pm0.17$ \\
56565 & $20.04\pm0.37$  & 56540 & $18.64\pm0.17$ \\
56590 & $20.59\pm0.25$  & 56541 & $18.65\pm0.18$ \\
56603 & $20.36\pm0.42$  & 56544 & $18.79\pm0.19$ \\
56841 & $21.00\pm0.14$  & 56546 & $18.77\pm0.18$ \\
56846 & $20.92\pm0.11$  & 56554 & $19.14\pm0.23$ \\
56862 & $21.12\pm0.22$  & 56558 & $18.72\pm0.14$ \\
56866 & $21.32\pm0.34$  & 56563 & $18.85\pm0.19$ \\
      &                 & 56565 & $18.80\pm0.26$ \\
      &                 & 56579 & $18.89\pm0.28$ \\
      &                 & 56584 & $18.88\pm0.18$ \\
      &                 & 56590 & $18.77\pm0.18$ \\
      &                 & 56603 & $18.89\pm0.24$ \\
      &                 & 56611 & $19.11\pm0.28$ \\
      &                 & 56616 & $18.86\pm0.31$ \\
      &                 & 56621 & $19.03\pm0.18$ \\
      &                 & 56639 & $18.95\pm0.35$ \\
      &                 & 56647 & $18.97\pm0.23$ \\
      &                 & 56814 & $19.48\pm0.14$ \\
      &                 & 56841 & $19.58\pm0.11$ \\
      &                 & 56843 & $19.38\pm0.14$ \\
      &                 & 56849 & $19.68\pm0.16$ \\
      &                 & 56853 & $19.75\pm0.32$ \\
      &                 & 56862 & $19.60\pm0.13$ \\
      &                 & 56866 & $19.75\pm0.09$ \\
      &                 & 56873 & $19.51\pm0.16$ \\
      &                 & 56893 & $19.84\pm0.43$ \\
      &                 & 56901 & $19.55\pm0.14$ \\
      &                 & 56917 & $20.02\pm0.12$ \\
      &                 & 56934 & $19.86\pm0.17$ \\
      &                 & 56967 & $20.17\pm0.26$ \\
      &                 & 56982 & $19.86\pm0.19$ \\
      &                 & 56991 & $20.03\pm0.33$ \\
      &                 & 57007 & $19.74\pm0.12$ \\
\hline
\multicolumn{2}{c}{LRIS $g$-band} & \multicolumn{2}{c}{LRIS $r$-band}\\
MJD & Magnitude & MJD & Magnitude \\
56981 & $21.4\pm0.20$ & 56981 & $20.0\pm0.20$ \\
\hline
\end{tabular}
\caption{Photometry of SN\,2009ip.}
\end{table}

